Two formalisms of stochastization of one-step models

To construct realistic mathematical models from the first principles, the authors suggest using the stochastization method. In a number of works different approaches to stochastization of mathematical models were considered. In the end, the whole variety of approaches was reduced to two formalisms: combinatorial (state vectors) and operator (occupation numbers). In the article the authors briefly describe these formalisms with an emphasis on their practical application.

==> bib/gen-sdu/Makefile <==
all: opt

opt:
	sed -i -e "s:^\([[:space:]]*\)url =:\1OPTurl =:g" *.bib
	sed -i -e "s:^\([[:space:]]*\)issn =:\1OPTissn =:g" *.bib
	sed -i -e "s:^\([[:space:]]*\)isbn =:\1OPTisbn =:g" *.bib


